Generative Models for the Deformation of Industrial Shapes with Linear Geometric Constraints: model order and parameter space reductions

Real-world applications of computational fluid dynamics often involve the evaluation of quantities of interest for several distinct geometries that define the computational domain or are embedded inside it. For example, design optimization studies require the realization of response surfaces from the parameters that determine the geometrical deformations to relevant outputs to be optimized. In this context, a crucial aspect to be addressed are the limited resources at disposal to computationally generate different geometries or to physically obtain them from direct measurements. This is the case for patient-specific biomedical applications for example. When additional linear geometrical constraints need to be imposed, the computational costs increase substantially. Such constraints include total volume conservation, barycenter location and fixed moments of inertia. We develop a new paradigm that employs generative models from machine learning to efficiently sample new geometries with linear constraints. A consequence of our approach is the reduction of the parameter space from the original geometrical parametrization to a low-dimensional latent space of the generative models. Crucial is the assessment of the quality of the distribution of the constrained geometries obtained with respect to physical and geometrical quantities of interest. Non-intrusive model order reduction is enhanced since smaller parametric spaces are considered. We test our methodology on two academic test cases: a mixed Poisson problem on the 3d Stanford bunny with fixed barycenter deformations and the multiphase turbulent incompressible Navier-Stokes equations for the Duisburg test case with fixed volume deformations of the naval hull.

==> sections/generative.tex <==
Generative models (GMs) have been successfully applied for computer graphics' tasks such as 3d objects generation. Their employment in surrogate modelling is especially beneficial when the computational costs needed to create a new geometry from real observations is reduced. One disadvantage is that depending on the complexity of the distribution to be approximated, their training requires a large amount of data. In this work, we focus on studying the possible employment of GMs for the reduction of the space of the parameters that specify geometrical deformations. In our case, the parameters are the displacements of cFFD. Another objective is to reduce the computational costs needed to generate new linear constrained geometries with cFFD.\TODO{add refs of GMs applied for ML tasks.}

We denote with $p_{X}(x)$ the probability density of the distribution of 3d objects and with $X:(A, \mathcal{A}, P)\rightarrow\mathbb{R}^{M}$ the random variable representing it, with $M$ the number of points or degrees of freedom of the 3d mesh. The triple $(A, \mathcal{A}, P)$ corresponds to the space of events, sigma algebra and probability measure of our setting. The variable $x$ may represent 3d point clouds, 3d meshes or general subdomains of $\mathbb{R}^3$. We are going to focus on generative models that approximate $p_{X}(x)$ with $p_{\theta}(x)$ where $\theta$ are parameters to be found and that can be factorized through latent variables $z$ such that 
\begin{equation}
    p_{\theta}(x)=\int_{Z} p_{\theta}(x|z)p_{\theta}(z)dz
\end{equation}
where $z$ is typically low dimensional with respect to $x$, with dimension $R\ll M$. These models are called latent variable models\cite{tomzack}.
Given a set of training samples of the distribution associated with $X$ obtained with cFFD (section~\ref{subsec:cffd}), the objective is to sample new 3d objects with quality comparable to the one generated using cFFD. It is crucial that the new samples satisfy exactly the linear or multilinear constraints imposed with cFFD.

As the subject of generative models is well-known in the literature we summarize briefly the architectures we are going to employ.

\paragraph{Simple Autoencoder}
As a toy model for pure benchmarking we first implement a very simple Autoencoder \cite{ae}, composed of two parts: an Encoder $Enc_{\psi}:\mathbb{R}^{M}\rightarrow \mathbb{R}^{R}$ which encodes the mesh in the latent space, and a Decoder $Dec_{\theta}: \mathbb{R}^{R} \rightarrow \mathbb{R}^{M}$ that takes a point of the latent space and returns it to the data space. 
Autoencoders were originally created for learning the latent representations of the data and have many applications \cite{ae}, like denoising. Some recent research has empirically shown  \cite{ghose,daly} that they can indeed be used as generative models.
They are trained on the $L^2$ loss
\begin{equation}
    L_{\theta,\psi}(x)=||x-Dec_{\theta}(Enc_{\psi}(x))||_{2},
\end{equation}
the associated generative model is
\begin{equation}
    p_{\theta}(x|z)=Dec_{\theta}(z)
\end{equation}
where $z$ is sampled from a multivariate normal distribution.

\paragraph{Beta Variational Autoencoder}
A Variational Autoencoder \cite{varauto} is a probabilistic version of the autoencoder. It is based on the concept of Evidence Variational Lower Bound (ELBO) that can be employed in place of the log-likelihood $p_{\theta}(x)$ when it is not directly computable. Given a variational distribution $q_{\psi}(z|x)$ the ELBO is 

\begin{equation}
    ELBO_{\psi,\theta}(x)= E_{q_\phi(z \mid x)}\left[\log \left(\frac{p_\theta(x, z)}{q_\phi(z \mid x)}\right)\right]= E_{q_\phi(z \mid x)}\left[\log \left(p_\theta(x \mid z)\right)\right]-K L\left(q_\phi(z \mid x) \| p_\theta(z)\right)
\end{equation}
it follows that
\begin{equation}
    ELBO_{\psi,\theta}(x)\le \log p_{\theta}(x).
\end{equation}

Variational autoencoders model $q_{\psi}(z|x)$ and $p_{\theta}(x|z)$ as two normal distributions:
\begin{equation}
    q_{\psi}(z|x)=\mathcal{N}(a_{\psi}(x),b_{\psi}(x))
\end{equation}
where $a_{\psi},b_{\psi}:\mathbb{R}^{M}\rightarrow \mathbb{R}^{R}$ are encoders and
\begin{equation}
    p_{\theta}(x|z)=\mathcal{N}(Dec_{\theta}(z),\sigma),
\end{equation}
Notice that, the $KL$ term in the ELBO is a regularizing term on the variational distribution.
Depending on the strength of $p_{\theta}(x|z)$ the Variational autoencoders can suffer from two problems: if it is dominant then there is no regularizing effect and so the samples from $p_{\theta}(z)$ will have poor quality. Otherwise, the $KL$ will go to $0$, so $a_{\psi},b_{\psi}$ will degenerate to constants and the model will start behaving autoregressively. To solve these two problems, an $\alpha$ term is added to the ELBO:
\begin{equation}
    L_{\theta,\phi}=E_{q_\phi(z \mid x)}\left[\log \left(p_\theta(x \mid z)\right)\right]-\alpha K L\left(q_\phi(z \mid x) \| p_\theta(z)\right),
\end{equation}
this technique is also used in \cite{qtan}.

\paragraph{Adversarial Autoencoder}
Another class of Generative Models is Generative Adversarial Networks which have the same structure of an autoencoder
\begin{equation}
    p_{\theta}(x|z)=Dec_{\theta}(z)
\end{equation} 
but they are trained with the help of a discriminator $D_{\lambda}$ in the following min-max game:
\begin{equation}
    \min _\theta \max _\lambda V(\theta, \lambda)=E_{p_X(x)}\left[\log \left(D_\lambda(x)\right)\right]+E_{p_\theta(z)}\left[\log \left(1-D_\lambda\left(Dec_\theta(z)\right)\right)\right].
\end{equation}
In this context, the decoder is also called generator.
The discriminator is used to distinguish between the data and the generator samples while the generator wants to fool it. A problem of generative adversarial networks is that the min-max game can bring instabilities, for the details of this we refer to \cite{arjovsky}. A solution is to combine them with variational autoencoders to get the following loss:
\begin{equation}
    \max _{\theta, \phi} \min _\lambda L_{\theta, \phi, \lambda}=E_{q_\phi(z, x)}\left[\log \left(p_\theta(x \mid z)\right)\right]-
E_{p_\theta(z)}\left[\log \left(1-D_\lambda(z)\right)\right]+E_{q_\phi(z)}\left[\log \left(D_\lambda(z)\right)\right],
\end{equation}
which is the ELBO with the GAN loss instead of the KL term.
This model is called Adversarial Autoencoder \cite{aae}. The associated generative model is
\begin{equation}
    p_{\theta}(x|z)=\mathcal{N}(Dec_{\theta}(z),\sigma), \quad\text{with}\quad z\sim\mathcal{N}(0, I_R)
\end{equation}

\paragraph{Boundary Equilibrium GAN}
Another solution to the GAN problems is the Boundary Equilibrium GAN \cite{began}. In this particular model, the discriminator is an autoencoder
\begin{equation}
    D_{\lambda}(x)=Dec_{\lambda}(Enc_{\lambda}(x))
\end{equation}
and the objective is to learn the autoencoder loss function
\begin{equation}
    f_{\lambda}=||x-D_{\lambda}(x)||_{2}
\end{equation}
while maintaining a balance between the data loss and the generator loss to prevent instabilities caused by the min-max training. Let $G_{\theta}$ the generator, this is achieved in three steps using control theory:
\begin{itemize}
    \item Solve $\min_{\lambda} E_{p_{X}(x)}[f_{\lambda}(x)]-k_{t} E_{p_{X}(x)}[f_{\lambda}(G_{\theta}(Enc_{\lambda}(x)))]$ over $\lambda$.
    \item Solve $\max_{\theta} E_{p_{Z}(z)}[f_{\lambda}(G_{\theta}(z)].$
    \item Update $k_{t}=k_{t-1}+a(\gamma E_{p_{X}(x)}[f_{\lambda}(x)]- E_{p_{Z}(z)}[f_{\lambda}(G_{\theta}(z)]).$
\end{itemize}

The associated generative model is
\begin{equation}
    p_{\theta}(x|z)=G_{\theta}(z), \quad\text{with}\quad z\sim\mathcal{N}(0, I_R).
\end{equation}

